Fundamental Limits of Nonintrusive Load Monitoring

Provided an arbitrary nonintrusive load monitoring (NILM) algorithm, we seek bounds on the probability of distinguishing between scenarios, given an aggregate power consumption signal. We introduce a framework for studying a general NILM algorithm, and analyze the theory in the general case. Then, we specialize to the case where the error is Gaussian. In both cases, we are able to derive upper bounds on the probability of distinguishing scenarios. Finally, we apply the results to real data to derive bounds on the probability of distinguishing between scenarios as a function of the measurement noise, the sampling rate, and the device usage.

==> backgroundHO.tex <==




The problem of NILM is essentially a single-channel source separation problem: determine the power consumption of individual devices given their aggregated power consumption. 
The source separation problem has a long history in information theory and signal processing and well known methods include the infomax principle \cite{Bell1995}, which tries to maximize some output entropy, the maximum likelihood principle \cite{Cardoso1997}, which uses a contrast function on some distribution on the source signals, and a time-coherence principle \cite{Belouchrani1997}, which assumes time-coherence of the underlying source signals. These often lead to formulations which use some variation of a principle components analysis (PCA) or independent component analysis (ICA).





The most common applications of the source separation theory is to audio signals and biomedical signals.  For these applications, it is often assumed that source signals are i.i.d.  stationary processes.  We note that power consumption signals are very different from these types of signals. The power consumption of a device has strong temporal correlations and are not stationary, e.g.~whether or not a device is on at a given time is correlated with whether or not it was on an instant ago, and the mean power consumption signal changes with the state of the device. %o such assumption makes sense here. {\bf WHY???}
The algorithmic and theoretical development in source separation have therefore not been successfully applied to NILM and most methods for NILM are rather different to those developed for classical source separation. 



The field of NILM is much younger than source separation and most  development has focused on algorithms. 
Most algorithms are batch algorithms and produce an estimate of the disaggregated signals given a batch of aggregate recordings.  
Broadly speaking, existing methods for NILM can be divided into two main approaches, namely, supervised and unsupervised. Supervised disaggregation methods require a disaggregated data set for training. This data set could be obtained by, for example, monitoring typical appliances using plug sensors. 
Supervised methods assume that the variations between signatures for the same type of appliances is less than that between signatures of different types of appliances. Hence, the disaggregated data set does not need to be from the building that the supervised algorithm is designed for. However, the disaggregated data set must be collected prior to deployment, and come from appliances of a similar type to those in the target building. Supervised methods are typically discriminative. The existing supervised methods include sparse coding \cite{Kolter2010}, change detection and clustering based approaches \cite{drenker1999:rk,rahayu2012:sk},  pattern recognition \cite{farinaccio1999:lk} and adaptive filtering \cite{Dong2013,Dong2013a}. The sparse coding approach tries to reconstruct the aggregate signal by selecting as few signatures as possible from a library of typical signatures. Similarly, in our previously proposed framework we construct a library of dynamical models and reconstruct the aggregate signal by using as few as possible of these models using well established methods from the filtering community.  




Unsupervised methods, on the other hand, do not require a disaggregated data set to be collected. They do, however, require hand tuning of parameters, which can make it hard for the methods to be generalized in practice. It should be said that also supervised methods have tuning parameters, but these can often be tuned using the training data. The existing unsupervised methods include factorial hidden Markov models (HMMs), difference hidden Markov models and variants \cite{kim11,Kolter2012,Johnson2012,parson2012:AAAI:lk,pattem2012:gk} and temporal motif mining \cite{Shao2012}. Most unsupervised  methods model the on/off sequences of appliances using some variation of HMMs. These methods do not directly make use of the signature of a device and assume that the power consumption is piecewise constant. For more on algorithms for NILM see e.g. \cite{Zeifman2011:fh} or \cite{Kolter2011}. 








The discussion  presented in this paper focus on the theoretical limitations of NILM. To the best of our knowledge, there has not been any previous work attempting to model the NILM problem in its full generality and derive theoretical bounds. The work is inspired  by recent work in differential privacy \cite{Dwork2006, Ny2012}. The underlying goal of differential privacy is to model privacy in a fashion that encapsulates arbitrary prior information on the part of the adversary and an arbitrary definition of what constitutes a privacy breach. 
The theory of differential privacy can be extended to give similar, but weaker, bounds to those derived in this paper. 


==> backgroundRD.tex <==
In recent years, the advent of AMIs has renewed interest in NIALM methods. In this section, we provide a review of the previous literature. First, we'll provide a quick overview of some work on NIALM.

There have been several public datasets published for the purposes of evaluation and comparison of NIALM algorithms. We describe a few of them now. %We describe some of these quickly here. 
One of the datasets is the Reference Energy Disaggregation Dataset (REDD) \cite{Kolter2011}, which provides the aggregate power consumption signal measured at the mains, as well as the plug-level power consumption signals for several houses. In contrast, there is the Building Level fUlly-labelled dataset for Energy Disaggregation (BLUED) \cite{Anderson2012}, which provides the aggregate power consumption signal as well as complete labels on when all devices switch states, such as when fans and lights turn on and off, or devices are activated. Additionally, there is the Smart* data set \cite{Barker2012}, which provides environmental data and motion sensor data as well as power consumption data.

We mention these datasets because the difference in the datasets emphasizes a philosophical point of this paper: many approaches are built around different ends, and even require different datasets for evaluation. REDD and BLUED are designed for energy disaggregation and event detection, respectively. The Smart* data set was not collected for any particular NIALM approach, but can be used for determining which exogenous factors are relevant to NIALM algorithms.

In additional to a variety of goals, there have been a variety of approaches. We outline some of them now.

One approach has focused on the design of hardware to best detect the signatures of distinct devices \cite{Leeb1995,Gupta2010,Froehlich2011}. This work has many exciting results, and even allows us to distinguish between two of the same light-bulb, if they are plugged into different outlets. However, it is still an open problem as to how to acquire labeled data to link the detected signatures to certain devices, as some of the results exploit small differences in the wiring of individual houses.

Another approach which has been done by much of the machine learning community is to use hidden Markov models (HMMs), or some variation, to model individual devices \cite{Kolter2011,Kolter2012,Parson2012}. These assume the device has an underlying latent state, whose dynamics are governed by a Markov chain. The observed output of each device comes from a distribution, often Gaussian, which depends only on the latent state. Finally, the aggregate output is the sum of the outputs of each of these HMMs.

These methods have a tractable expectation-maximization (EM) algorithm that is well studied in the literature and often, in theory, they do not require a disaggregated data set for training. However, in practice, a disaggregated data set is often required for the tuning of priors. Additionally, there are many devices whose power consumption dynamics do not satisfy the Markov assumptions; some work has been done to relax this with hidden semi-Markov models and sticky hidden Markov models \cite{Johnson2012}. There still remains work to be done on how to find good priors and tuning parameters for these relaxations.

In recent publications \cite{Dong2013,Dong2013a}, we also introduced a novel framework for understanding the energy disaggregation problem. We required a training dataset from which we can learn models for the dynamics of the devices, as well as a prior on the device usage patterns of consumers. Then, we phrased the goal of energy disaggregation as finding the maximum a posteriori (MAP) estimate of the device usage given the observed aggregate signal. We were able to leverage results from adaptive filtering and provide a recursive algorithm amenable to online deployment with theoretical guarantees on when it recovers the MAP solution. However, it is still an open problem how to interact with unmodeled devices in the aggregate signal, as well as the best methods to identify device dynamics and device usage profiles.

In summary, there is a lot of work currently being done on NIALM, but the problem is far from solved. 
In this paper, our goal is to provide a general theoretic framework for analyzing the efficacy and fundamental limits of all of these approaches. 
To the best of our knowledge, there has not been any previous work attempting to model the NIALM problem in its full generality and derive theoretical bounds. 
As mentioned in Section \ref{sec:introduction}, these fundamental limits could be used to determine minimal specifications for AMIs that which to achieve a certain goal, as well as provide guarantees of privacy for policy-makers. 

\subsection{Connections with source separation literature}
In this section, we compare our formulations in this paper to existing literature on the source separation problem.

The problem of NIALM can be thought of as a single-channel source separation problem: the current power meters and many smart meters only measure the aggregate power consumption signal, which is the result of coupling of the outputs of many devices. 

A source separation problem is one where sensors measure mixtures of a set of signals, which are not known in advance. This problem is, in general, ill-posed, and %Because of the lack of knowledge of the source signals, 
the chief problem of source separation is the formulation and implementation of some principle for evaluating the quality of source signals. 

Several principles have been studied before, such as the infomax principle \cite{Bell1995}, which tries to maximize some output entropy, the maximum likelihood principle \cite{Cardoso1997}, which uses a contrast function on some distribution on the source signals, and a time-coherence principle \cite{Belouchrani1997}, which assumes time-coherence of the underlying source signals. These often lead to formulations which use some variation of a principle components analysis (PCA) or independent component analysis (ICA).

However, much of this work utilizes the fact that there are multiple sensors. The single-channel source separation has been studied less extensively, likely because the topic is much more application-specific. Some references include \cite{Jang2003,Mijovic2010}.
%In \cite{Jang2003}, the authors extend the maximum likelihood principle to the single-channel source separation problem, and \cite{Mijovic2010} investigates a single-channel source separation problem with application to biomedical signals.

The most common applications of the source separation theory is to audio signals and biomedical signals. We note that power consumption signals are very different from these types of signals. Often, the work in the past has assumed the source signals are i.i.d. stationary processes. No such assumption makes sense here. In contrast, some of the other work which uses basis functions can be likened to the frameworks presented in our previous work \cite{Dong2013,Dong2013a}; however, many NIALM approaches do not assume such basis functions.

We believe that the problem of NIALM, although a single-channel source separation problem, is very distinct from the previous work done on the topic, and this paper can be seen as a first step in the study of this particular class of single-channel source separation problems.

